Comparing Visual Reasoning in Humans and AI

Recent advances in natural language processing and computer vision have led to AI models that interpret simple scenes at human levels. Yet, we do not have a complete understanding of how humans and AI models differ in their interpretation of more complex scenes. We created a dataset of complex scenes that contained human behaviors and social interactions. AI and humans had to describe the scenes with a sentence. We used a quantitative metric of similarity between scene descriptions of the AI/human and ground truth of five other human descriptions of each scene. Results show that the machine/human agreement scene descriptions are much lower than human/human agreement for our complex scenes. Using an experimental manipulation that occludes different spatial regions of the scenes, we assessed how machines and humans vary in utilizing regions of images to understand the scenes. Together, our results are a first step toward understanding how machines fall short of human visual reasoning with complex scenes depicting human behaviors.

==> leftover.tex <==
\subsection{Are the same regions important for Humans and OSCAR?}
 We computed the correlation between Humans and OSCAR for the masked BERTScores (relative to the corresponding unmasked descriptions) across mask positions for each image. We also computed the correlation between humans by dividing the masked human data into two groups. Fig.\ref{fig:MaskCorrPlots} shows that the effect of mask position on the descriptions for each image has higher correlation within humans than for humans with OSCAR

\begin{figure}[!hbt]
    \centering
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Fig4a.jpeg}
         \caption{}
         \label{fig:HVsOmaskCorr}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Fig4b.jpeg}
         \caption{}
         \label{fig:HVsHmaskCorr}
    \end{subfigure}
    \caption{Histogram of Correlation of BERTScores across masked positions}
    \label{fig:MaskCorrPlots}
\end{figure}

 We compared human and OSCAR's descriptions for the masked images  to their corresponding unmasked descriptions
 
 
 \subsubsection*{Acknowledgments}
The research was funded by the U.S. Army Research Office under Contract Number W911NF-19-D-0001 for the Institute for Collaborative Biotechnologies.  The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation herein. 
